Kernelization of Counting Problems

We introduce a new framework for the analysis of preprocessing routines for parameterized counting problems. Existing frameworks that encapsulate parameterized counting problems permit the usage of exponential (rather than polynomial) time either explicitly or by implicitly reducing the counting problems to enumeration problems. Thus, our framework is the only one in the spirit of classic kernelization (as well as lossy kernelization). Specifically, we define a compression of a counting problem $P$ into a counting problem $Q$ as a pair of polynomial-time procedures: $\mathsf{reduce}$ and $\mathsf{lift}$. Given an instance of $P$, $\mathsf{reduce}$ outputs an instance of $Q$ whose size is bounded by a function $f$ of the parameter, and given the number of solutions to the instance of $Q$, $\mathsf{lift}$ outputs the number of solutions to the instance of $P$. When $P=Q$, compression is termed kernelization, and when $f$ is polynomial, compression is termed polynomial compression. Our technical (and other conceptual) contributions concern both upper bounds and lower bounds.

==> conclusion.tex <==
%!TEX root = mainCountingKernelization.tex

\section{Conclusion}\label{sec:conclusion}

\hly{TODO}

==> preamble.tex <==
%!TEX root = mainDiskGraphs.tex

\newcommand{\longversion}[1]{{#1}
\newcommand{\shortversion}[1]}

\usepackage[dvipsnames,svgnames,x11names]{xcolor}
\usepackage{amssymb,amsmath,mathrsfs}
\usepackage{soul}
\usepackage{mathtools}
\usepackage{framed}
\usepackage{mdframed}
\usepackage{tcolorbox}
\usepackage{amsmath}

\newcommand{\hlr}[1]{\sethlcolor{Salmon1}\hl{#1}\sethlcolor{yellow}} 
\newcommand{\hlg}[1]{\sethlcolor{PaleGreen2}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlb}[1]{\sethlcolor{SkyBlue1}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hlo}[1]{\sethlcolor{Apricot}\hl{#1}\sethlcolor{yellow}}
\newcommand{\hly}[1]{\sethlcolor{Gold}\hl{#1}\sethlcolor{yellow}}

\usepackage{listings}
\usepackage{mathrsfs}
\usepackage[mathscr]{euscript}
\usepackage{amsfonts,amsthm,amsmath}
\usepackage{amstext}
\usepackage{graphicx,tikz}
\RequirePackage{fancyhdr}
\usepackage{boxedminipage}
\usepackage{todonotes}
\usepackage[linesnumbered, boxed, algosection,noline]{algorithm2e}
\usepackage{graphics}
\usepackage{framed}
\usepackage{thm-restate}
\usepackage{thmtools}
\usepackage{enumerate}
\usepackage{float}
\usepackage{xspace}
\usepackage{thm-restate}
%\usepackage{todonotes}

\newcommand{\OO}{\mathcal{O}}
\newcommand{\cO}{\mathcal{O}}

\usepackage{vmargin}
\setmarginsrb{2cm}{2cm}{2cm}{2cm}{0pt}{0pt}{0pt}{6mm}

\newcommand{\myparagraph}[1]{\smallskip\noindent{\textbf{\sffamily #1}}}

\newtheorem{theorem}{Theorem}%[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{claim}[lemma]{Claim}
\newtheorem{corollary}[lemma]{Corollary}
\newtheorem{definition}[lemma]{Definition}
\newtheorem{observation}[lemma]{Observation}
\newtheorem{proposition}[lemma]{Proposition}
\newtheorem{redrule}[lemma]{Reduction Rule}
\newtheorem{remark}[lemma]{Remark}
\newtheorem{reduction}[lemma]{Reduction Rule}
\newtheorem{conjecture}[lemma]{Conjecture}
\newtheorem{fact}[lemma]{Fact}

\mathchardef\myhyphen="2D
 
\newcommand{\defparproblem}[4]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1  & {\bf{Parameter:}} #3 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #4
  \end{minipage}
}\vspace{1mm}}

\newcommand{\defproblem}[3]{
\vspace{1mm}
\noindent\fbox{
  \begin{minipage}{0.96\textwidth}
  \begin{tabular*}{\textwidth}{@{\extracolsep{\fill}}lr} #1 \\ \end{tabular*}
  {\bf{Input:}} #2  \\
  {\bf{Question:}} #3
  \end{minipage}
}\vspace{1mm}}

\usepackage{booktabs}
\usepackage[pdftex, plainpages = false, pdfpagelabels, 
                 %pdfpagelayout = useoutlines,
                 bookmarks=false,
                 bookmarksopen = true,
                 bookmarksnumbered = true,
                 breaklinks = true,
                 linktocpage,
                 pagebackref,
                 colorlinks = true,  % was true
                 linkcolor = blue,
                 urlcolor  = blue,
                 citecolor = red,
                 anchorcolor = green,
                 hyperindex = true,
                 hyperfigures
                 ]{hyperref}

% general
\newcommand{\yes}{\textsf{Yes}}
\newcommand{\no}{\textsf{No}}
\newcommand{\yesinstance}{\yes-instance}
\newcommand{\noinstance}{\no-instance}
\newcommand{\tw}{\mathtt{tw}}
\newcommand{\equ}{\mathtt{Equiv}}
\newcommand{\NP}{\textsf{NP}}
\newcommand{\coNP}{\textsf{co-NP}}
\newcommand{\FPT}{\textsf{FPT}}
\newcommand{\XP}{\text{XP}}
\newcommand{\WO}{\textsf{W[1]}}
\newcommand{\WOH}{\textsf{W[1]}-hard}
\newcommand{\WOC}{\textsf{W[1]}-complete}
\newcommand{\WTH}{\textsf{W[2]}-hard}
\newcommand{\WTC}{\textsf{W[2]}-complete}
\newcommand{\NPH}{\textsf{NP}-hard}
\newcommand{\NPC}{\textsf{NP}-complete}
\newcommand{\paraH}{\textsf{para-NP}-hard}
\newcommand{\ETH}{\textsf{ETH}}
\newcommand{\SETH}{\textsf{SETH}}
\newcommand{\alg}{\textsf{ALG}}
\newcommand{\nil}{\ensuremath{\mathtt{nil}}}
\newcommand{\dist}{\ensuremath{\mathsf{dist}}}
\newcommand{\flow}{\ensuremath{\mathsf{Flow}}}
\newcommand{\cupdot}{\mathbin{\mathaccent\cdot\cup}}
\newcommand{\paths}{\mbox{\sf Paths}}

%Problem Name

\usepackage{xspace}
\newcommand{\pname}{\textsc}
\newcommand{\ProblemFormat}[1]{\pname{#1}}
\newcommand{\ProblemIndex}[1]{\index{problem!\ProblemFormat{#1}}}
\newcommand{\ProblemName}[1]{\ProblemFormat{#1}\ProblemIndex{#1}{}\xspace}

\newcommand{\probPVD}{\ProblemName{Planar Vertex Deletion}}
\newcommand{\probCVD}{\ProblemName{Chordal Vertex Deletion}}
\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
\newcommand{\probEMC}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probGFVS}{\ProblemName{Group Feedback Vertex Set}}
\newcommand{\probEMultiC}{\ProblemName{Edge Multicut}}
\newcommand{\probSFVS}{\ProblemName{Subset Feedback Vertex Set}}
\newcommand{\probTWdel}{\ProblemName{Treewidth-$\eta$ Modulator}}
\newcommand{\probFdel}{\ProblemName{$\mathcal{F}$-Deletion}}
\newcommand{\probFpack}{\ProblemName{$\mathcal{F}$-Packing}}
\newcommand{\probSdel}{\ProblemName{$\mathcal{S}$-Deletion}}
\newcommand{\probSpack}{\ProblemName{$\mathcal{S}$-Packing}}
% Commonly used names
\newcommand{\probVC}{\ProblemName{Vertex Cover}}
\newcommand{\probPlVC}{\ProblemName{Planar Vertex Cover}}
\newcommand{\probPVC}{\ProblemName{Partial Vertex Cover}}
\newcommand{\probPDS}{\ProblemName{Partial Dominating Set}}
\newcommand{\probPrDS}{\ProblemName{Partial $r$-Dominating Set}}
\newcommand{\probFVS}{\ProblemName{Feedback Vertex Set}}
\newcommand{\probIFVS}{\ProblemName{Independent Feedback Vertex Set}}
\newcommand{\probCycPacking}{\ProblemName{Cycle Packing}}
\newcommand{\probPlFVS}{\ProblemName{Planar Feedback Vertex Set}}
\newcommand{\probIS}{\ProblemName{Independent Set}}
\newcommand{\probWIS}{\ProblemName{Weighted Independent Set}}
\newcommand{\probMCIS}{\ProblemName{Multicolored Independent Set}}
\newcommand{\probDS}{\ProblemName{Dominating Set}}
\newcommand{\probrDS}{\ProblemName{$r$-Dominating Set}}
\newcommand{\probrSC}{\ProblemName{$r$-Scattered Set}}
%\newcommand{\probMDS}{\ProblemName{Minimum Dominating Set}}
\newcommand{\probPlDS}{\ProblemName{Planar Dominating Set}}
\newcommand{\probCDS}{\ProblemName{Connected Dominating Set}}
\newcommand{\probDST}{\ProblemName{Dominating Set on Tournaments}}
\newcommand{\probClique}{\ProblemName{Clique}}
\newcommand{\probMC}{\ProblemName{Multicolored Clique}}
\newcommand{\probPClique}{\ProblemName{Partitioned Clique}}
\newcommand{\probqSC}{\ProblemName{$q$-Set Cover}}
\newcommand{\probSC}{\ProblemName{Set Cover}}
\newcommand{\probDSP}{\ProblemName{Dominating Set with Pattern}}
%\newcommand{\probOCT}{\ProblemName{Odd Cycle Transversal}}
%\newcommand{\probEB}{\ProblemName{Edge Bipartization}}
\newcommand{\probHam}{\ProblemName{Hamiltonian Cycle}}
\newcommand{\probPlHam}{\ProblemName{Planar Hamiltonian Cycle}}
\newcommand{\probHamP}{\ProblemName{Hamiltonian Path}}
\newcommand{\probKPath}{\ProblemName{Longest Path}}
\newcommand{\probWKPath}{\ProblemName{Weighted Longest Path}}
\newcommand{\probthreeSAT}{\ProblemName{$3$-SAT}}
\newcommand{\probqSAT}{\ProblemName{$q$-SAT}}
\newcommand{\probcnfSAT}{\ProblemName{CNF-SAT}}
\newcommand{\probthreeCol}{\ProblemName{$3$-Coloring}}
\newcommand{\probqCol}{\ProblemName{$q$-Coloring}}
\newcommand{\probListColoring}{\ProblemName{List Coloring}}
\newcommand{\probOddSet}{\ProblemName{Odd Set}}
\newcommand{\probTuring}{\ProblemName{Short Turing Machine Acceptance}}
\newcommand{\probSI}{\ProblemName{Subgraph Isomorphism}}
\newcommand{\probGI}{\ProblemName{Graph Isomorphism}}
\newcommand{\probWCS}{\ProblemName{Weighted Circuit Satisfiability}}
\newcommand{\probClosestString}{\ProblemName{Closest String}}
\newcommand{\probClosestSubstring}{\ProblemName{Closest Substring}}
\newcommand{\probGridTiling}{\ProblemName{Grid Tiling}}
\newcommand{\probGridTilingLeq}{\ProblemName{Grid Tiling with~$\le$}}
\newcommand{\probUnitDisk}{\ProblemName{Unit Disk Independent Set}}
\newcommand{\probEMWay}{\ProblemName{Edge Multiway Cut}}
\newcommand{\probEDS}{\ProblemName{Edge Dominating Set}}
\newcommand{\probEMWaySets}{\ProblemName{Edge Multiway Cut for Sets}}
\newcommand{\probDirEMWay}{\ProblemName{Directed Edge Multiway Cut}}
\newcommand{\probEMCut}{\ProblemName{Edge Multicut}}
\newcommand{\probMulticut}{\ProblemName{Multicut}}
\newcommand{\probDirEMCut}{\ProblemName{Directed Edge Multicut}}
\newcommand{\probSkewEMCut}{\ProblemName{Skew Edge Multicut}}
\newcommand{\probDFVS}{\ProblemName{Directed Feedback Vertex Set}}
\newcommand{\probDFAS}{\ProblemName{Directed Feedback Arc Set}}
\newcommand{\probDFASC}{\ProblemName{Directed Feedback Arc Set Compression}}
\newcommand{\probPartpq}{\ProblemName{$(p,q)$-Partition}}
\newcommand{\probClusterpq}{\ProblemName{$(p,q)$-Cluster}}
\newcommand{\probSatellite}{\ProblemName{Satellite Problem}}
\newcommand{\probTw}{\ProblemName{Treewidth}}
\newcommand{\probPerfSetMatch}{\ProblemName{Perfect $d$-Set Matching}}
\newcommand{\probHS}{\ProblemName{Hitting Set}}
\newcommand{\probdHS}{\ProblemName{$d$-Hitting Set}}
\newcommand{\probEdHS}{\ProblemName{E$d$-Hitting Set}}
\newcommand{\probSetSplit}{\ProblemName{Set Splitting}}
\newcommand{\probSteiner}{\ProblemName{Steiner Tree}}
\newcommand{\probSteinerF}{\ProblemName{Steiner Forest}}
\newcommand{\probMotif}{\ProblemName{Graph Motif}}
\newcommand{\probColorfulMotif}{\ProblemName{Colorful Graph Motif}}
\newcommand{\probRBDSlong}{\ProblemName{Red-Blue Dominating Set}}
\newcommand{\probRBDS}{\ProblemNameX{RBDS}{Red-Blue Dominating Set}}
\newcommand{\probCRBDSlong}{\ProblemName{Colored Red-Blue Dominating Set}}
\newcommand{\probCRBDS}{\ProblemNameX{Col-RBDS}{Colored Red-Blue Dominating Set}}
\newcommand{\probCVC}{\ProblemName{Connected Vertex Cover}}
\newcommand{\probCFVS}{\ProblemName{Connected Feedback Vertex Set}}
\newcommand{\probCBullHit}{\ProblemName{Connected Bull Hitting}}
\newcommand{\probSetPacking}{\ProblemName{Set Packing}}
\newcommand{\probDisFactors}{\ProblemName{Disjoint Factors}}
\newcommand{\probDisPaths}{\ProblemName{Vertex Disjoint Paths}}
\newcommand{\probChromatic}{\ProblemName{Chromatic Number}}
\newcommand{\probECC}{\ProblemName{Edge Clique Cover}}
\newcommand{\probSubsetSum}{\ProblemName{Subset Sum}}
\newcommand{\probKnapsack}{\ProblemName{Knapsack}}
\newcommand{\probWayCut}{\ProblemName{$s$-Way Cut}}
\newcommand{\probEulerian}{\ProblemName{Eulerian  Deletion}}
\newcommand{\probBisec}{\ProblemName{Minimum Bisection}}
\newcommand{\probMaxBisec}{\ProblemName{Maximum Bisection}}

% specific
\newcommand{\disk}{\ensuremath{\mathsf{disk}}}
\newcommand{\obj}{\ensuremath{\mathsf{obj}}}
\newcommand{\rel}{\ensuremath{\mathsf{relevant}}}
\newcommand{\cri}{\ensuremath{\mathsf{critical}}}
\newcommand{\dis}{\ensuremath{\mathsf{distance}}}
\newcommand{\ft}{\ensuremath{\mathsf{FTR}}}
\newcommand{\unc}{\ensuremath{\mathsf{uncontract}}}
\newcommand{\ori}{\ensuremath{\mathsf{origin}}}

